Cooperation Networks: Endogeneity and Complexity

Insights from the Complex Systems literature are employed to develop a computational model of truly endogenous strategic network formation. Artificial Adaptive Agents, implemented as Finite State Automata (FSA), play a modified two-player IPD game with an option to further develop the interaction space as part of their strategy. Several insights result from this minor modification: first, I find that network formation is a necessary condition for cooperation to be sustainable but that both the frequency of interaction and the degree to which edge formation impacts agent mixing are both necessary conditions for cooperative networks. Second, within the FSA-modified IPD frame-work, a rich ecology of agents and network topologies is observed and described. Third, the system dynamics are investigated and reveal that initially simple dynamics with small interaction length between agents gives way to complex, a-periodic dynamics with self-organized critical properties when interaction lengths are increased by a single step.

==> parts/ga_expl.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%     file : 0408_trustnets/ga_expl.tex
%   author : S. Angus
% creation : 27 Oct 05
%

\subsubsection*{Crossover Operator}

In this model, the crossover operator represents learning by imitation. It is 
assumed that new agents enter the population after having witnessed the 
behaviour of the incumbent elites, and so enter having copied part or all of 
these successful strategies.

The crossover operator (Fig.~\ref{fg:crossover}) is extremely simple to apply: 
two agent bit-strings from the elite population are selected at random; at some 
uniform random point along each string, a `cut' is made\footnote{This is the 
so-called `one-point' crossover operator, other versions include `two-point', 
`three-point' and so on.}, and the two trailing pieces are switched, thus 
forming two `new' agents (assuming there is at least one difference in these two 
pieces) from the strategies of the `old' agents.

%%% FIGURE: figs/misc/crossover.fig
\fighere{fg:crossover}

It is important to note that the `cut-point' is selected at random along the 
string length. In this way, after successive `generations' of play, successful 
portions of each strategy will be replicated and amplified in the new 
population. Such accumulation of strategic insight over time speaks directly 
to real-life technology adoption or behavioural learning. However, attention 
is drawn to the fact that in this framework, the new population's technology 
accumulation content is contingent entirely on the previous period's 
population only. There is little facility here (except consistency between 
periods, or chance) for the new population to replicate exactly portions of 
successful strategies from several or more periods previous to the current 
one.\footnote{%
	One may also care to notice that although the cut-point is uniform random, 
	the probability that a given bit will be `switched' in the crossover 
	operation is not. Infact, for some bit at position $a$, with string length 
	$L$, the probability that $a$ will undergo crossover is $\frac{a}{L}$.  
	Thus, in this formulation, bits to the left (start) of the string are least 
	likely to undergo crossover, whilst those to the right (end) of the string 
	are most likely. Hence, the initial strategy state is more likely to be 
	retained between elite and new agent, with subsequent states more likely to 
	undergo switching.}


\subsubsection*{Mutuation Operator}

Following application of the crossover operator, each new agent bit string 
undergoes a mutation operator. Simply put, with low (independent) probability (1 
or 5\%) each bit in the string is `flipped': $0 \ra 1$; or $1 \ra 0$ (see 
Fig.~\ref{fg:mutation}). For example, at the 1\% and 5\% levels, a six state 
strategy (66 bit) would undergo approximately $<1$ and 3 bit `flips' 
respectively.

%%% FIGURE: figs/misc/mutation.fig
\fighere{fg:mutation}

Such flipping is akin to the `mistake making', or `trembling hand' 
interpretation elsewhere in the strategic literature.  In the current context, 
it represents either imperfect imitation/learning from successful incumbents, or 
self-driven innovation by entrants. Regardless, its random strategy generation, 
taken together with the non-random selection mechanism, provide an opportunity 
for the population to evolve in a positive manner. Successful components of new 
strategies are rewarded with more followers in future populations, whilst 
unsuccessful agents leave, making way for fresh entrants.




==> parts/measures.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%     file : 0408_trustnets/measures.tex
%   author : S. Angus
% creation : 27 Oct 05
%

\begin{description}

\item[Age, $\langle age \rangle$]
The average age of each agent-node in a cluster. It is to be noted that there 
will be much inter-temporal dependance in this data, since a cluster of some set 
of agents will `age' together over time.
\item[Payoff by Period, $\langle \Pi_{period} \rangle$]
Average node total payoff in each `period' for a cluster. Inter-period selection 
of `elites' is based on this measure.
\item[Payoff by Interaction, $\langle \Pi_{int} \rangle$]
Average node payoff for the individual iterations of the PD. This is a measure 
of cooperation/defection events for agents. It is to be noted that if two 
$Cagent$s play together, then they will receive $\{3,3\}$. Depending on their 
strategies, either they will obtain 1 the rest of the time \{D,D\} or 0 in the 
case that they play $C$ to an opponent's $D$.

If interactions are only ever in two types: `within' the network between two 
$Cagents$, play then being $C$,\verb=#(s)=, or `outside' the network between 
a $Cagent$ and a foreign ($D$-playing agent), play for the $Cagent$ then being 
$C$, $D$ (the most `intelligent' of the strategies), the proportion of 
`inside'/`outside' interactions for each agent in the network can be found, 
since the interaction payoff will be a weighted sum of the `inside' events 
together with the `outside' events.
\[
	\langle\Pi_{int}\rangle = \alpha(inside: 3) + (1-\alpha)(outside: 1)
\]
Implies that,
\[
	\alpha = \frac{\langle\Pi_{int}\rangle - 1}{2}
\]
For example, if $\langle\Pi_{int}\rangle = 2.6$ then $\alpha = 0.8$. That is, 
agents in these clusters interact, on average, 80\% of the time with other 
$Cagent$ network agents.
\item[Clustering Coefficient, $C$] Following~\cite{118_Wat_col}, a measure of 
the degree of local-connectedness in a graph. It uses the theoretical number of 
edges between an adjacency set of nodes and determines what fraction the real 
incidence of such nodes comprises. Thus, $0 \leq C \leq 1$. For a regular random 
graph $\mathcal{R}$ of degree $k$ and size $n$,
\[
	C(\mathcal{R}) \sim \frac{k}{n}.
\]
\item[Char. Path Length, $L$] Again, following Watts and Strogatz~\cite{118_Wat_col}, $L$ is the average minimum path length (hops) between each node in a connected graph. For a regular random graph $\mathcal{R}$ of degree $k$ and size $n$,
\[
	L(\mathcal{R}) \sim \frac{ln(n)}{ln(k)}.
\]
\item[Degree, $\langle D \rangle$]
Simply the average degree of each agent-node in the graph.
\item[Cluster Size, $\langle N \rangle$]
The number of nodes in the connected component.
\end{description}




==> parts/proof_mutual.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%     file : 0408_trustnets/proof_mutual.tex
%   author : S. Angus
% creation : 27 Oct 05
%

\begin{rem}
Under mutual stopping conditions, when $\k=2$ and $k=4$, the strategy quadruple 
$s^{u,m}_{D}: \{D,D,D,D\}$ is the only evolutionary stable strategy.
\end{rem}
\begin{proof}{}
We begin in the same manner as above, however, in this case, we will not specify 
the successful strategy immediately. Specifically, suppose that two strategies 
of the form $s^{u,m}: \{P_{1},R(C),R(D),R(\#)\}$ are labeled $s^{u,m}_{X}$ and 
$s^{u,m}_{S}$ for convenience. Now again, let $\alpha$ be the proportion of type 
$\mbf{S}$ in the population. We proceed as before, constructing the ESS strategy 
$s^{u,m}_{X}$ by considering requirements for stability once the strategy is 
established, and infiltration, if another strategy is established.

Now suppose $\alpha = 0$, then if $\mbf{X}$ is to be stable from attack by any 
$\mbf{S}$ then,
\begin{equation}\label{eq:mutalph0}
	\Pi(\mbf{X}|\mbf{X}) \geq \Pi(\mbf{S}|\mbf{X})
\end{equation}
which by substitution as in Remark~\ref{rm:uinlateral} becomes,
\[
	\G(P^{X}_{1}|P^{X}_{1}) + \G(R^{X}(P^{X}_{1})|R^{X}(P^{X}_{1}))
	\geq \G(P^{S}_{1}|P^{X}_{1}) + \G(R^{S}(P^{X}_{1})|R^{X}(P^{S}_{1})).
\]
We note that if $P^{X}_{1} = P^{S}_{1} = P_{1}$ then this implies that,
\begin{equation}\label{eq:pssame}
	\G(R^{X}(P_{1})|R^{X}(P_{1})) \geq \G(R^{S}(P_{1})|R^{X}(P_{1})).
\end{equation}
It can be seen that the LHS of \eqref{eq:pssame} is on the principal diagonal 
of $\G$ whereas the RHS is unconstrained. We note that if, and only if, 
$R^{X}(P_{1}) = C$, equation~\eqref{eq:pssame} will not hold, therefore, 
$R^{X}(P_{1}) \in \{D,\#\}$.

Now suppose that $P^{X}_{1} \neq P^{S}_{1}$ and that $P^{X}_{1}=C$, then 
\eqref{eq:mutalph0} is,
\begin{equation}\label{eq:blue}
	3 + \G(R^{X}(C)|R^{X}(C))
	\geq \G(P^{S}_{1}|C) + \G(R^{S}(C)|R^{X}(P^{S}_{1})).
\end{equation}
However, an unconstrained payoff of 5 is available to $\mbf{S}$ in the first 
iteration, which implies that unless $\G(R^{X}(P^{X}_{1})|R^{X}(P^{X}_{1})) 
= 3$ (the mutual cooperative outcome), \eqref{eq:blue} will not hold, but 
since $R^{X}(P_{1}) \in \{D,\#\}$ this is impossible, hence, $P^{X}_{1} \neq 
C$.

Turning to the $\alpha = 1$ case, if $\mbf{X}$ is to infiltrate any strategy 
$S$ then,
\begin{equation}\label{eq:mut1domcond}
	\Pi(\mbf{X}|\mbf{S}) \geq \Pi(\mbf{S}|\mbf{S}),
\end{equation}
which becomes, 
\begin{equation}\label{eq:red}
	\G(P^{X}_{1}|P^{S}_{1}) + \G(R^{X}(P^{S}_{1})|R^{S}(P^{X}_{1}))
	\geq \G(P^{S}_{1}|P^{S}_{1}) + \G(R^{S}(P^{S}_{1})|R^{S}(P^{S}_{1})).
\end{equation}
Now, suppose $P^{X}_{1} = \#$, then the above condition reduces to,
\[
	\G(R^{X}(P^{S}_{1})|R^{S}(P^{X}_{1}))
	\geq \G(R^{S}(P^{S}_{1})|R^{S}(P^{S}_{1}))
\]
which is not true for all $P^{S}_{1}$ and $R^{S}(P_{1})$ (for example, 
$P^{S}_{1}=C$ and $R^{S}(C)=C$), hence, $P^{X}_{1} \neq \#$. Therefore, allow 
$P^{X}_{1} = D$ and note that $\max(RHS~\eqref{eq:red})=6$, then 
$\G(R^{X}(P^{S}_{1})|R^{S}(P^{X}_{1})) \geq 1$. However, if $R^{S}(D) = \#$ 
this will not be true. Hence, there is one strategy that is stable to attack 
from the current built strategy namely, $s^{u,m}_{S}: \{C,C,\#,\dots\}$.  
However, $s^{u,m}_{S}$ does not fulfill the conditions given above for stable 
strategies ($\alpha = 0$), and can be successfully invaded by $s^{u,m}_{M}: 
\{C,D,D,D\}$.  Therefore, we can conclude that there is no viably stable 
strategy that will withstand attack from a variant comprising the elements,
\[
	s^{u,m}_{X*}: \{D,\{D,\#\},\{D,\#\},\{D,\#\}\}
\]
Finally, we note that for any response to an opponent's play, $D$ weakly 
dominates $\#$ and hence, the strategy,
\[
	s^{u,m}_{X}: \{D,D,D,D\}
\]
will be preferred.
\end{proof}


